Accuracy to Throughput Trade-offs for Reduced Precision Neural Networks on Reconfigurable Logic

Modern CNN are typically based on floating point linear algebra based implementations. Recently, reduced precision NN have been gaining popularity as they require significantly less memory and computational resources compared to floating point. This is particularly important in power constrained compute environments. However, in many cases a reduction in precision comes at a small cost to the accuracy of the resultant network. In this work, we investigate the accuracy-throughput trade-off for various parameter precision applied to different types of NN models. We firstly propose a quantization training strategy that allows reduced precision NN inference with a lower memory footprint and competitive model accuracy. Then, we quantitatively formulate the relationship between data representation and hardware efficiency. Our experiments finally provide insightful observation. For example, one of our tests show 32-bit floating point is more hardware efficient than 1-bit parameters to achieve 99% MNIST accuracy. In general, 2-bit and 4-bit fixed point parameters show better hardware trade-off on small-scale datasets like MNIST and CIFAR-10 while 4-bit provide the best trade-off in large-scale tasks like AlexNet on ImageNet dataset within our tested problem domain.

==> 2-relatedwork.tex <==
\section{Related Works}
\label{related_work}

Parameter quantization is widely studied as an approach to explore model redundancy and reduce computation/memory challenges \cite{gupta15}\cite{lin16}. For such approaches, a neural network with high-precision parameters is preliminarily trained and the parameters are then quantized into low-precision substitutes for inference efficiency. \cite{lin16} proposed a layer-wise quantization method which is based on a Signal-to-Quantization-Noise Ratio (SQNR) minimization. Meanwhile, Gupta \textit{et. al.} have shown that a combination of fixed-point representations for network parameters and a stochastic rounding strategy can achieve comparable training results with floating point representations while providing advantages of reduced computational complexity and improved power efficiency \cite{gupta15}. However, only 3 fixed-point representations are considered in their experiments. Above methods are mainly test-phase quantization strategies, which generally do not work very well with extremely low bitwidth, say 1 or 2 bits, because of the introduced quantization errors. 

To target this issue, training low-precision weights after direct quantization proves to be a practical technique to enhance model performance \cite{hwang1014}\cite{anwar15}\cite{ResiliencyUnderQuantization}. In these approaches, low-precision parameters are used for (feed-forward and backward) propagations and high-precision values for weight updating. This strategy is especially beneficial to high-throughput power-efficient inference engine design \cite{finn}\cite{intelbnn}. 

For example, in \cite{courbariaux0915}, dynamic fixed-point, fixed point and floating point representations are studied on different \gls{NN} models. This work is very similar to ours in terms of exploring different precisions and their impact on classification error. However, in our work, we further take into consideration system throughput (\gls{FPS}) and resource overhead which help to build a more comprehensive view of the benefits of low-precision numerals. We also cover the representation capability of extremely low bitwidth, while in \cite{courbariaux0915} the practical word length for fixed-point parameters can be no less than 20 bits. Lower bitwidth (10 bits) can be used for dynamic fixed-point solutions, which are not inherently supported by mainstream computing platforms on the hardware level. 

Recently, binary or ternary weights have been found sufficient to achieve similar or even better results than their floating point alternatives \cite{binarynet}\cite{tnn}\cite{lin0216}\cite{xnornet}. The introduction of such extremely low bitwidth representations can also convert the expensive multiplications between weights and neuron activations into simple XNOR and popcount operations. In addition significant memory can be saved for parameter storage \cite{finn}.

Although the above-mentioned works have dedicated great efforts on unveiling the benefits of using reduced precision parameters, they can not provide answers to the following questions: to achieve a specific classification accuracy for a given model and dataset, what precision of parameters can deliver the highest inference throughput (\gls{FPS})? For accuracy purpose, is it worthy to apply lower precision but higher amount of parameters for NNs in terms hardware cost and inference throughput?

We strive to address above questions by systematically exploring the relationship between parameter precision and system performance and network size and topology. In this work, networks are trained with weights and activations separately represented by Binary, 2-bit, 4-bit, 8-bit, 16-bit fixed point and single-precision floating point representations. Our aim is to provide insights into the architectural design of efficient inference systems on reconfigurable hardware.
